Low-rank Tensor Learning with Nonconvex Overlapped Nuclear Norm Regularization

Nonconvex regularization has been popularly used in low-rank matrix learning. However, extending it for low-rank tensor learning is still computationally expensive. To address this problem, we develop an efficient solver for use with a nonconvex extension of the overlapped nuclear norm regularizer. Based on the proximal average algorithm, the proposed algorithm can avoid expensive tensor folding/unfolding operations. A special "sparse plus low-rank" structure is maintained throughout the iterations, and allows fast computation of the individual proximal steps. Empirical convergence is further improved with the use of adaptive momentum. We provide convergence guarantees to critical points on smooth losses and also on objectives satisfying the Kurdyka-{\L}ojasiewicz condition. While the optimization problem is nonconvex and nonsmooth, we show that its critical points still have good statistical performance on the tensor completion problem. Experiments on various synthetic and real-world data sets show that the proposed algorithm is efficient in both time and space and more accurate than the existing state-of-the-art.

==> cover.tex <==
\begin{center}
	\Large\bf
	Cover Letter
\end{center}

\noindent
\section*{Dear Associate Editor:}

I would like to submit the following paper entitled 
``Efficient Low-rank Tensor Learning with Nonconvex Overlapped Nuclear Norm Regularization'' 
for consideration of publication in the JMLR.
This submission is 
encouraged to be revised and re-submitted.
The
previous summary is as follows.

\vspace{10px}
\noindent
\textbf{Summary.}
{\it
	The reviewers in general are positive about the paper. However, there are a couple of concerns
	that came into focus: 
	1). the main technique and contribution of the paper seems a bit incremental
	especially wrt work of Yao et al. Clarifying how the work relates to some of the existing results
	in the domain and also highlighting key technical challenges should strengthen the paper. 
	2). implications of the main theorem (Theorem 14) are not clear and further clarifications and
	connections to realistic problem settings would be helpful.}

\vspace{5px}
\noindent
\textbf{Reply.}
We strictly follow reviewers' suggestions and have fully revise the submission.
\begin{itemize}[leftmargin=*]
	\item 
	For 1):
	The difficulties of extending to higher order tensors
	are discussed after Proposition~\ref{pr:mulv};
	the meaning of nonsmooth loss and side-information,
	which previously confuses reviewers, 
	are clarified in the abstract, 
	introduction
	and Section~\ref{sec:extend}.
	
	\item 
	For 2):
	We limit our discussion to the tensor completion problem to make 
	implications of the main theorem more clear.
	We prove that tensors that are not too spiky can be recovered.
	Besides,
	we also show
	how the recovery performance can depend on
	noise level,
	tensor ranks,
	and the number of observations.
\end{itemize}
We hope the revision can well address concerns raised by previous reviewers.

\vspace{10px}
\noindent
I confirm that all co-authors are aware of the current submission and consent to its review by JMLR. 

\vspace{10px}
\noindent
Thank you for your kind consideration.

\vspace{10px}
\noindent
-- Quanming

==> reply.tex <==
\begin{center}
	\Large\bf
	Reply for ``{Efficient Low-rank Tensor Learning with
		Nonconvex Overlapped Nuclear Norm Regularization}''
\end{center}



\section*{To Reviewer \#1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q1.1.}
{\it
	The authors claim that one of the main contributions of the current paper is the
	statistical guarantee of the proposed method. However, the established result, i.e.,
	Theorem 14 (Theorem~\ref{thm:stat} in this revision), 
	is not very clear. What is $\kappa_0$ in the statement? Does it correspond to
	the parameter in Assumption 1? 
}

\vspace{5px}
\noindent
\textbf{Reply.}
Yes.
$\kappa_0$ corresponds to the parameter in Assumption~\ref{ass:kappa}.
We have added more explanations below Theorem~\ref{thm:stat}
(i.e., Theorem~14 in the old version)
to make above points clear.
%\footnote{$\surd$ *** will need to copy those new points here (when the main text is stable)}
For an easy reference,
we also copy the text here
\begin{itemize}[leftmargin=*]
\item Besides,
recall that $\kappa_0$ in Assumption~\ref{ass:kappa}
reflects how nonconvex the function $\kappa(\alpha)$ is; while
$\alpha_1$ in Definition~\ref{ass:rsc}
measures strong convexity.
Thus,
these two quantities play opposing roles in \eqref{eq:guarantee}.
Specifically,
a larger $\alpha_1$ leads to a larger $a_v$,
and subsequently smaller 
$\| \ten{X}^* - \tilde{\ten{X}} \|_F$; whereas a 
larger $\kappa_0$ leads to a larger $\frac{ \lambda \kappa_0 c_v }{a_v}$,
and subsequently larger 
$\| \ten{X}^* - \tilde{\ten{X}} \|_F$.
\end{itemize}


%\footnote{+qm+ more experiments need to be done}
%and new experiments in Section~\ref{sec:quacri} to show the impact of $\kappa_0$
%on the quality of critical points.

%\begin{center}
%\color{blue}
%Copy corresponding text here.
%\end{center}


%\begin{itemize}
%	\item see text under Theorem~2 in \cite{loh2015regularized},
%	add a remark on $(\alpha_1, \mu)$.
%\end{itemize}


\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q1.2.}
{\it
	Why the distance error given in this theorem is
	independent of number of observations $\| \Omega \|_1$?
}

\vspace{5px}
\noindent
\textbf{Reply.}
The error indeed decays as a rate of $O( 1 / \sqrt{\NM{\bm{\Omega}}{1}} )$
where $\NM{\bm{\Omega}}{1}$ is the number of observations.
In this revised version,
we make this dependency clear by
adding Corollary~\ref{cor:number}
in Section~\ref{sec:depobv}.
%(which follows from Theorem~\ref{thm:stat}). 
We also perform additional experiments in Section~\ref{sec:exp:obvnsy}.
In particular, Figure~\ref{fig:rmse:obv} 
demonstrates that the linear dependency in Corollary~\ref{cor:number}
can be empirically observed.

%\begin{itemize}
%	\item check text under (7) in~\citep{loh2015regularized},
%	re-do the proof by replacing
%	assumptions on $\lambda = c \sqrt{ \| \Omega \|_1 / (mn)}$
%	
%	\item perhaps, also need to add noisy ratio to the above $\lambda$.
%	See example in Corollary~3.6 in~\citep{gui2016towards}.
%\end{itemize}

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q2.}
\textit{Theorem 14 (Theorem~\ref{thm:stat} in this revision) 
	is based on the Restricted Strong Convexity (RSC) condition, i.e.,
	Assumption 2. Can the authors give several examples to show that RSC condition
	can indeed be satisfied for different low-rank tensor completion problems?}

\vspace{5px}
\noindent
\textbf{Reply.}
%Please check the new Section~\ref{sec:stat}.
In this revision,
we added Lemma~\ref{lem:rsc:hold}, which shows that when the number of
observations is sufficiently large,
the RSC condition holds when the low-rank tensor is not too spiky.

%we have limited our scope of statistical analysis to the tensor completion problem.  Then, we motivate what kind of tensors can be recovered in Section~\ref{sec:obvmod}.  Basically, low-rank tensors which are not spiky are more likely to be completed.  These help us establish Subsequently, we show how RSC can be met by the tensor completion in 


\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q3.}
\textit{The authors claim that the extended method can deal with the nonsmooth loss.
	However, Section 4.1 in the current paper only considers a specific form of nonsmooth loss. 
	Therefore, the author may want to tone down their contributions for
	nonsmooth loss or giving more examples to show that the current loss can cover a
	bunch of nonsmooth loss functions for low-rank tensor completion problems.}

\vspace{5px}
\noindent
\textbf{Reply.}
As suggested, instead of using the term
``\textit{using nonsmooth loss}'' which may be overly general, we now use the term 
%toned down claims on ``\textit{using nonsmooth loss}''.  Specifically, in this revision,
``robust loss".
relevant parts
in the abstract,
introduction,
and conclusion
are also changed.

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q4.}
\textit{The authors also claim that the proposed method can handle the side information.
	However, Section 4.1 in the current paper only considers a graph Laplacian regularized method. Thus, the authors should clarify their contributions in the introduction
	section.}

\vspace{5px}
\noindent
\textbf{Reply.}
As suggested, instead of using the term
``side information'', we now use the 
more specific 
``graph Laplacian Regularization''.
other revised parts are also changed.

\vspace{5px}
\hrule
\vspace{10px}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q5.}
\textit{For the synthetic data, it would be helpful if the authors can also study higher-order
	tensors instead of just 3rd order tensors to validate the effectiveness of the current
	method..}

\vspace{5px}
\noindent
\textbf{Reply.}
As suggested,
we have added such experiments in Section~\ref{sec:orderrank}.

\vspace{5px}
\hrule
\vspace{10px}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q6.}
\textit{To evaluate the statistical error of the proposed method, I would suggest the authors
	to plot the error versus the tensor order, rank, and number of observations.}

\vspace{5px}
\noindent
\textbf{Reply.}
As suggested,
we have added experiments on
the number of observations in Section~\ref{sec:exp:obvnsy},
and experiments on the tensor rank and order
in Section~\ref{sec:orderrank}.

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q7.}
\textit{There is a line of research \citep{zheng2015convergent,tu2016low,wang2017unified} studying the factorization based nonconvex
	low-rank matrix learning, and statistical guarantees of low-rank (robust) tensor
	decomposition~\citep{gu2014robust}, the authors may want to comment on these works in Section 2.1
	and Section 2.2.}

\vspace{5px}
\noindent
\textbf{Reply.}
These methods~\citep{zheng2015convergent,tu2016low,wang2017unified}
solve matrix completion problem based on the low-rank factorization approach,
then variants of gradient descent are used for optimization.
In this revised version,
we 
introduce these methods
in the new
Section~\ref{sec:matfact}.

%the suggested references are all included.

For RTDGC~\citep{gu2014robust},
it considers robust tensor decomposition 
with the convex overlapping nuclear norm 
%for low-rank
and 
$\ell_1$-loss.
We have included it in Section~\ref{sec:ten:reg} and Section~\ref{sec:robustc}
in this revision.
Besides,
in the previous version,
we compare with ADMM
in Section~\ref{sec:exp:rpca} for experiments on robust matrix completion.
Since RTDGC also uses standard ADMM for 
robust matrix completion,
we further make it clear that it is RTDGC that we are compared with.


%\begin{itemize}[leftmargin=*]
%\item 
%\footnote{+qm+ add in Section~\ref{sec:rel:nonreg}.
%	no need to add experimental comparison,
%	since factorization approach has already been considered in Table~\ref{tab:comparedalgs}.}
%
%\item \cite{gu2014robust} considers robust tensor decomposition 
%with convex overlapping nuclear norm 
%for low-rank
%and 
%$\ell_1$-norm 
%for sparsity.
%\footnote{+qm+ need to compare in Section~\ref{sec:exp:rpca},
%	add as convex approach in Table~\ref{tab:robust}.}
%\footnote{+qm+ need to add in Section~\ref{sec:robustc}.}
%\end{itemize}


\section*{To Reviewer \#2}

\subsubsection*{Questions on convergence guarantee}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q1.}
\textit{What additional difficulties does this additional folding/unfolding operations add to proving
	the convergence of the PA algorithm?}

\vspace{5px}
\noindent
\textbf{Reply.}
%As shown in Table~\ref{tab:overview},
The proposed algorithm has
two main differences
with existing 
PA algorithms for the nonconvex optimization problem
\eqref{eq:compopt}
(with a smooth loss function and nonconvex regularization):
(i) folding/unfolding operations, and
(ii) use of adaptive momentum.
%\footnote{+qm+ need to clarify  in the ``proof ideas''.}
The main difficulty in the convergence proof
is caused by point (ii),
in which we need to show 
how existing convergence proofs can be combined with the adaptive momentum.
This is why 
in the proof of Theorem~\ref{thm:conv} (Appendix~\ref{app:proof:thm:conv}),
we have two cases:
$\chi_1(\infty)$ and $\chi_2(\infty)$.
Next, we have to show
how the above proof 
is compatible with the additional folding/unfolding operations.
For example,
in \eqref{eq:app11},
we have to use 
$\langle \ten{Z}_{\ip{d}}, \bm{X}_{d} \rangle = \langle \ten{Z},
\bm{X}_{d}^{\ip{d}} \rangle$.


%For the classical proximal average operator~\citep{yu2013better,zhong2014gradient},
%we usually have that 
%there exists a function
%$g$ such that
%$\Px{g}{\bm{z}} = \sum_{i} \Px{g_1}{\bm{z}}$ for a vector $\bm{z}$.
%Note that,
%in this case,
%all $\Px{g_1}{\bm{z}}$'s have the same shape
%and they can be directly summed up.
%
%
%The main difficulty is to establish 
%Proposition~\ref{pr:reg} and~\ref{pr:bnd}.
%Specifically,
%comparing with 
%the classical proximal average operator above,
%our results is in form 
%of $\Px{ \nicefrac{ \bar{g}_{\tau} }{ \tau } }{\ten{Z}}
%=  \sum_{i = 1}^D [ \Px{ \nicefrac{\lambda_i \phi}{ \tau } }{ [ \ten{Z} ]_{\ip{i}} } ]^{ \ip{i} } $,
%where unfolding is performed before the proximal step
%and folding is performed after the proximal step.
%Thus,
%we need to show how folding/unfolding can pass the proof of 
%classical proximal average operator.
%See example in (\ref{eq:app16}),
%i.e.,
%how $\vect{X}_{d}^{\ip{d}}$ is transformed in $\vect{X}_{d}$.\footnote{*** i dont
%see how
%(\ref{eq:app16}) shows 
%"how $\vect{X}_{d}^{\ip{d}}$ is transformed in $\vect{X}_{d}$"? do u actually mean the
%step after
%(\ref{eq:app16})?
%\footnote{*** i think the part after
%"Specifically,..." above may just be removed}
%}
%
%Based on Proposition~\ref{pr:reg} and~\ref{pr:bnd},
%the convergence proof in Theorem~\ref{thm:conv},
%\ref{thm:rate}
%and \ref{thm:klrate}
%follows the classical proof routine
%in the optimization literature~\citep{zhong2014gradient,bolte2014proximal,yu2015minimizing,li2015accelerated,Li2017ada}.


%$g$ such that
%$\Px{g}{\bm{z}} = \sum_{i} \Px{g_1}{\bm{z}}$

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q2.}
\textit{Proposition 6 (Proposition~\ref{pr:reg} in this revision): Can you provide more details on what exactly does the $\bar{g}_\tau$ function
	look like?}

\vspace{5px}
\noindent
\textbf{Reply.}
In this revised version,
we added the following 
exact form of $\bar{g}_{\tau}$
in Proposition~\ref{pr:reg}:
\begin{align*}
\bar{g}_{\tau}(\ten{X})
= 
\tau
\big[ 
\min\nolimits_{ \{ \vect{X}_{d} \} } 
\sum\nolimits_{d = 1}^D 
\big( \frac{1}{2} \NM{\vect{X}_d}{F}^2 
+  \frac{\lambda_d}{\tau} \phi (\vect{X}_d) \big)
- \frac{D}{2}\NM{ \ten{X} }{F}^2
\text{\;s.t.\;} 
\sum\nolimits_{d = 1}^D \vect{X}_{d}^{\ip{d}} = \ten{X}
\big].
\end{align*}

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q3.}
\textit{Proposition 7 (Proposition~\ref{pr:bnd} in this revision): What is the relation between the critical points of $F$ and $F_\tau$?}

\vspace{5px}
\noindent
\textbf{Reply.}
There is no direct relationship between
an arbitrary critical point of 
$F_\tau$ and 
an arbitrary critical point of 
$F$.
However,
this Proposition 
(Proposition~\ref{pr:bnd} in the revised version)
shows the minimum of $F_\tau$
can serve as
an approximation to the minimum of $F$.
Thus,
by finding critical points of 
$F_\tau$,
we hope a good solution to $F_\tau$
can also be found.

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q4.}
\textit{Proposition 8 (Proposition~\ref{pr:criti} in this revision): For completeness, it would be useful to provide a proof of this in the appendix?}

\vspace{5px}
\noindent
\textbf{Reply.}
As suggested, 
the proof has been added in Appendix~\ref{app:pr:criti}.
%Proposition~\ref{pr:criti} in the revised version
%\footnote{+qm+ to be added.}

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q5.1.}
\textit{Theorem 9 (Theorem~\ref{thm:conv} in this revision): I think this theorem warrants a more detailed discussion, especially a proof sketch
	or idea of why this is the case.}

\vspace{5px}
\noindent
\textbf{Reply.}
%\footnote{+qm+ this is the standard statement of convergence result,
%	i.e., e.g., Theorem 1 in \citep{li2015accelerated}.}
As suggested,
we have added a proof sketch.
%right after Theorem~\ref{thm:conv}.
The main idea is as follows.
First,
we show  that
\begin{itemize}[leftmargin=*]
		\item If step~5 is performed,
	$F_{\tau}(\ten{X}_{t + 1})
	\le  F_{\tau}(\ten{X}_t)  -  \frac{\eta}{2}\NM{\ten{X}_{t + 1}  -  \bar{\ten{X}}_t}{F}^2$.
	
	\item If step~7 is performed, we have
	$F_{\tau}(\ten{X}_{t + 1})
	\le F_{\tau}(\ten{X}_t)
	- \frac{\eta}{2}\NM{\ten{X}_{t + 1} - \ten{X}_t}{F}^2$.
\end{itemize}
Combining the above two conditions,
we obtain
\begin{align*}
	\frac{2}{\eta} ( F_{\tau}(\ten{X}_1) - F_{\tau}(\ten{X}_{T + 1}) )
	\ge 
	\sum\nolimits_{j \in \chi_1(T)} 
	\NM{\ten{X}_{t + 1} - \bar{\ten{X}}_t}{F}^2
	+  \sum\nolimits_{j \in \chi_2(T)} \NM{\ten{X}_{t + 1} - \ten{X}_t}{F}^2,
\end{align*}
where $(\chi_1(T),\chi_2(T))$ is a partition of $\{ 1, \dots, T \}$
such that 
when $j \in \chi_1(T)$ 
step~5 is performed,
and 
step~7 is performed
when $j \in \chi_2(T)$.
Finally,
when $T \rightarrow \infty$,
we discuss three cases:
(i) $\chi_1(\infty)$ is finite, $\chi_2(\infty)$ is infinite;
(ii) $\chi_1(\infty)$ is infinite, $\chi_2(\infty)$ is finite; and
(iii) both $\chi_1(\infty)$ and $\chi_2(\infty)$ are infinite.
Let $\ten{X}_*$ be a limit point of $\{ \ten{X}_t \}$,
and $\{ \ten{X}_{j_t} \}$ be a subsequence that converges to $\ten{X}_*$.
In all the three cases,
we show  that
\begin{align*}
\lim\limits_{j_t \rightarrow \infty} \NM{\ten{X}_{j_t + 1} - \ten{X}_{j_t}}{F}^2
=
\| 
\Px{\nicefrac{\bar{g}_{\tau}}{\tau}}{\ten{X}_{*} - \frac{1}{\tau} \nabla
f(\ten{X}_{*})} - \ten{X}_{*} 
\|_F^2 = 0.
\end{align*}
Thus,
$\ten{X}^*$ is also a critical point 
based on Proposition~\ref{pr:criti}.
It is easy to see that
we have not made any specifications
on the limit points.
Thus, all limit points are also critical points.

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q5.2.}
\textit{Further, is this relation only one way -- that is, can there
	exist limits points of the algorithm which are not critical points of $F_\tau$?}

\vspace{5px}
\noindent
\textbf{Reply.}
All limit points are critical points,
please see our reply for Q5.1 above.
%and there are no outliers.
%Moreover,
%please note
%that this 
%statement 
%on critical points
%is fairly standard  in 
%many convergence results
%(e.g., 
%Theorem 1 in~\citep{wright2009sparse},
%Theorem 1 in~\citep{gong2013general},
%and Theorem 1 in~\citep{li2015accelerated}).



\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q6.}
\textit{
	I think overall this section can be improved a lot by providing more intuition and explanations
	around the various theorems and propositions informing the reader what the result is and also
	giving a short description of the proof idea.}

\vspace{5px}
\noindent
\textbf{Reply.}
As suggested,
we have revised the manuscript and
clarified the connections among the
various theoretical results.
We have also added a summary paragraph at the beginning of Section~\ref{sec:convana}. 
Basically,
there
are three general steps to show the convergence of
the PA algorithm~\citep{yu2013better,zhong2014gradient,yu2015minimizing}:
\begin{itemize}[leftmargin=*]
	\item Showing that there exists
	a new regularizer that 
	the proximal average step with $g_i$'s in \eqref{eq:proxavg3}
	attempts to solve (Proposition~\ref{pr:reg}).
	
	\item
	Showing  that
	the new regularizer, when combined with 
	the loss $f$ in \eqref{eq:compopt},
	serves as a good approximation to 
	the original objective $F$
	(Proposition~\ref{pr:bnd}). 
	
	\item
	Showing that
	the proposed algorithm
	finds critical points of the approximated optimization problem
	(Theorems~\ref{thm:conv} and \ref{thm:klrate}).
\end{itemize} 
We have also 
added a proof sketch to Theorem~\ref{thm:klrate},
and
changed
the statements around those 
Propositions and Theorems to make their connections clearer.

\subsubsection*{Questions on statistical guarantees}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q7.}
\textit{It would be useful to specify the precise incoherence condition and compare it with the RSC
	condition for completeness.}

\vspace{5px}
\noindent
\textbf{Reply.}
In 
Section~\ref{ssec:rsc} of 
this revised version,
we added one paragraph 
to summarize the differences between
RSC and incoherence.
%However, since the detailed description for the matrix incoherent condition is beyond the focus of the main text, we elaborate what precisely is 
More details 
%on incoherence and the reasons why RSC is less restrictive than incoherent are discussed 
can be found in 
Appendix~\ref{app:incoh}.

%We have added 
%more descriptions in Section~\ref{ssec:rsc}
%and a detailed comparison in 
%\footnote{+qm+ add.}
%Appendix~\ref{app:incoh}.
%\footnote{+qm+ copy Section~3.4.2 in \citep{negahban2012restricted} here?}

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q8.1.}
\textit{This section studies the statistical properties of the first-order critical points, but does not
	detail the observation model. In particular, are the entries in $\Omega$ sampled i.i.d.? }

\vspace{5px}
\noindent
\textbf{Reply.}
In this revised version,
we add the observation model at the beginning of Section~\ref{sec:obvmod}.
Specifically, entries in $\Omega$ are sampled i.i.d.
In Section~\ref{ssec:rsc},
we 
then
require that the sample operator follows
the RSC condition.
%In Lemma~\ref{lem:rsc:hold}, we show how low-rank tensors that are not spiky meet the RSC condition.

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q8.2.}
\textit{Are
	these observations noisy (from the theorem statement, it appears not)? As in the experiments, it
	would be useful to prove a version of Theorem 14 
	(Theorem~\ref{thm:stat} in this revision)
	with noise added to the observations, to make it
	statistical in nature.}

\vspace{5px}
\noindent
\textbf{Reply.}
In the previous version, we only impose the RSC condition on $\SO{\cdot}$, and Theorem~\ref{thm:stat} does not explicitly show the dependency on the noise level.
In 
this revised version,
we explicitly 
assume
additive noise 
in Section~\ref{sec:depobv}.
%and then derive Corollary~\ref{cor:noisy} and Theorem~\ref{thm:stat}.
Experimental results 
are also added 
in Section~\ref{sec:exp:obvnsy}
to illustrate this dependency. 

%\footnote{+qm+ check experiments.}
%From Figure~\ref{fig:noisy}, we can see that the error can be very small when the noisy level is zero, and the error increases linearly as with $\sigma$ gets larger.

%Specifically, we show that the dependency on noise level is in this form \begin{align*} \big\| \ten{X}^* - \tilde{\ten{X}} \big\|_F \le \sigma \frac{ b_2 \kappa_0 c_v }{a_v} \sum\nolimits_{i = 1}^M  \sqrt{k_i}.  \end{align*}

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q9.}
\textit{Theorem 14 (Theorem~\ref{thm:stat} in this revision) assumes that $\lambda$ satisfies a certain condition -- is such a $\lambda$ always
	guaranteed to exist? If not, then what does the theorem have to say about those cases?}

\vspace{5px}
\noindent
\textbf{Reply.}
No,
such a $\lambda$ may not always exist.
When it does not exist,
it usually indicates the tensor completion problem is too hard to get a good recovery performance.
To understand when this can happen,
consider the two extreme cases:
\begin{itemize}[leftmargin=20px]
\item[C1.]
There is no noise in the observations,
i.e.,
$\SO{\ten{X}^* - \ten{O}}$ 
$ = 0$.
In this case, 
(\ref{eq:lambda}) reduces to 
\begin{align*} 
\frac{4 \alpha_2}{\kappa_0}
\sqrt{ \log I^{\pi} / \NM{\vect{\Omega}}{1} }
\le
\lambda
\le
\frac{\alpha_2}{ 4 R \kappa_0 }.
\end{align*}
Thus,
such a $\lambda$ may not exist
when the number of observations, i.e., $\NM{\bm{\Omega}}{1}$, 
is too small.

%%This can be empirically observed .
%Take the curve of GDPAN/NORT with $\sigma = 10^{-5}$ in Figure~\ref{fig:rmse:obv} as an example.
%We can see that when $\sqrt{\log(I^{\pi}) / \NM{\bm{\Omega}}{1}}$
%% ($\NM{\bm{\Omega}}{1}$ is large)
%is small (e.g., $0.001$),
%the testing RMSE is very small (nearly zero).
%However,
%the testing RMSE already becomes very bad, 
%when $\sqrt{\log(I^{\pi}) / \NM{\bm{\Omega}}{1}}$ is large (e.g., $0.016$).
%%We can further expec
%\footnote{$\surd$ 
%	I mean if $\NM{\Omega}{1}$ is too small 
%	such that 
%	$\frac{4 \alpha_2}{\kappa_0}
%	\sqrt{ \log I^{\pi} / \NM{\vect{\Omega}}{1} }
%	>
%	\frac{\alpha_2}{ 4 R \kappa_0 }$,
%	then no $\lambda$ can exist.
%	Then,
%	in this case,
%	the performance can be very bad due to too few observations.
%	*** so what u're saying is that the rmse should be small even when 
%	$\sqrt{\log(I^{\pi}) / \NM{\bm{\Omega}}{1}}=0.016$, right? 
%	and then u argue that
%	it's because
%	$\lambda$ does not exist. but it's a bit hard to say. the q is: when there're
%	very few obser, should one expect zero testing rmse when data has no noise?
%	indeed, in 1st para of sec3.5.1, u argue that recovery can be very hard if u hv
%	too few obs. though u hv somehow avoided spiky tensors in ur analysis, this
%	problem may still exist? ***
%	$\surd$
%	the problem is not how it depends on $\sigma$.
%	Here,
%	I want to emphasize
%	the recovery performance is bad
%	when $\lambda$ does not exists,
%	since it means
%	the noisy level is too high or the observation is too few.
%	*** u mean the linear dep no longer
%	holds? but that contradicts w/ ur coro 3.15 (which should hold for small enough
%	$\sigma$). in particular, in the footnote there u said that the $\lambda$ in 
%	cor 3.15 does satisfy the bnd}
%Thus,
%with too small $\NM{\bm{\Omega}}{1}$
%such that 
%$\frac{4 \alpha_2}{\kappa_0}
%\sqrt{ \log I^{\pi} / \NM{\vect{\Omega}}{1} }
%>
%\frac{\alpha_2}{ 4 R \kappa_0 }$,
%then no $\lambda$ can exist,
%the recovery performance can be bad. 

\item [C2.]
All elements are observed,
then 
we have
$\alpha_1 = \alpha_2 = 1$ and $\tau_1 = \tau_2 = 0$ in Definition~\ref{ass:rsc}
due to
$\NM{ \SO{ \Delta } }{F}^2 = \NM{ \Delta }{F}^2$.
Besides,
the noise is not too small,
which means
$\sqrt{ \log I^{\pi} / \NM{\vect{\Omega}}{1} } \le \max_i 
\|  \left[ \ten{X}^* - \ten{O} \right]_{\ip{i}} \|_{\infty}$.
Then, 
(\ref{eq:lambda}) reduces to 
\begin{align*} 
	\frac{4}{\kappa_0}
	\max_{i} \| \left[ \ten{X}^* - \ten{O} \right]_{\ip{i}} \|_{\infty}
	\le
	\lambda
	\le
	\frac{\alpha_2}{ 4 R \kappa_0 }.
\end{align*}
Thus,
such a $\lambda$ may not exist when the noise is too high.

%Take the curve of GDPAN/NORT with $s = 62.5\%$ in Figure~\ref{fig:rmse:noisy}
%as an example.
%We can see that 
%the recovery performance is already bad when $\sigma = 10^{-1}$,
%and when $\sigma$ gets larger,
%i.e.,
%$\max_{i} \| \left[ \ten{X}^* - \ten{O} \right]_{\ip{i}} \|_{\infty}$ 
%becomes larger,
%the performance can get even worse.
%This
%again indicates when the $\lambda$ does not exists,
%the recovery performance can be bad.
%\footnote{$\surd$ see the above.
%	*** why is this a problem? as u said in cor3.15, the err increases linearly w/ $\sigma$}
\end{itemize}
We have also added the above to Section~\ref{sec:mainrst}.

%To simplify the discussion,
%consider the two extreme cases:
%\begin{itemize}
%\item[C1.]
%There is no noise in the observations,
%i.e.,
%$\SO{\ten{X}^* - \ten{O}}$ 
%$ = 0$.
%In this case,
%the condition in Theorem~\ref{thm:stat} reduces
%to 
%\begin{align*} 
%\sqrt{ \log I^{\pi} / \NM{\bm{\Omega}}{1} }
%\le
%\lambda
%\le 1 / (16 R).
%\end{align*}
%Thus,
%%given a fixed $R$,
%such a $\lambda$ may not exist
%when the number of observations, i.e., $\NM{\bm{\Omega}}{1}$, 
%is too small.
%
%
%\item [C2.]
%All elements are observed and noise is not too small.
%In this case,
%we have $\alpha_1 = \alpha_2 = 1$, 
%$\tau_1 = \tau_2 = 0$, 
%and $\sqrt{ \log I^{\pi} / \NM{\vect{\Omega}}{1} } \le \max_i 
%\|  \left[ \SO{ \ten{X}^* - \ten{O} } \right]_{\ip{i}} \|_{\infty}$,
%then the condition in Theorem~\ref{thm:stat} reduces
%to 
%\begin{align*} 
%\max_i 
%\left\|  \left[ \SO{ \ten{X}^* - \ten{O} } \right]_{\ip{i}} \right\|_{\infty}
%\le
%\lambda
%\le
%1 / (16 R).
%\end{align*}
%Thus,
%%given a fixed $R$,
%such a $\lambda$ may not exist when the noise is too high.
%%\footnote{+qm+ need to update a new figure.}
%
%\end{itemize}


\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q10.}
\textit{Can the authors explain a bit about the infinity norm condition on the first order critical
	point that is required to hold in theorem 14 (Theorem~\ref{thm:stat} in this revision)? 
	Why is the scaling on the infinity
	norm required to be less than $\lambda \cdot \kappa_0$?}

\vspace{5px}
\noindent
\textbf{Reply.}
In this revision,
we improved the proof 
and this assumption is no longer needed.
Specifically,
in the previous version,
the infinity norm condition 
is used in
(68):
\begin{align*}
\left\langle 
\partial r(\tilde{\ten{X}}) + \nabla f \left( \ten{X}^* \right),
\tilde{\ten{V}}
\right\rangle 
\le \min_i
\Big( 
\| [\nabla f ( \tilde{ \ten{X} } )]_{\ip{i}} \|_{\infty} 
+
\| [\nabla f \left( \ten{X}^* \right)]_{\ip{i}} \|_{\infty} 
\Big) 
\tilde{v}_i
%\label{rpy:bnd}
\end{align*}
to bound $\| [\nabla f ( \tilde{ \ten{X} } )]_{\ip{i}} \|_{\infty} $.
In \eqref{eq:temp2} of 
this revised version,
we adopt a different strategy to expand the LHS of the above inequality, as:
\begin{eqnarray*}
\langle
\partial r(\tilde{\ten{X}}) + \nabla f \left( \ten{X}^* \right),
\tilde{\ten{V}}
\rangle 
&
= & 
\langle
\nabla f \left( \ten{X}^* \right),
\tilde{\ten{V}}
\rangle 
+
\lambda \sum\nolimits_{i = 1}^D 
\langle
\partial \phi( \ten{X}_{\ip{i}} ),
\tilde{\ten{V}}_{\ip{i}}
\rangle,
\nonumber \\
& 
\le & \max_i
\left\| [\nabla f \left( \ten{X}^* \right)]_{\ip{i}} \right\|_{\infty} \tilde{v}_i
+
\lambda \sum\nolimits_{i = 1}^D 
\left\| \partial \phi( \ten{X}_{\ip{i}} ) \right\|_{\infty} \tilde{v}_i.
\end{eqnarray*}
The term
$\left\| [\nabla f \left( \ten{X}^* \right)]_{\ip{i}} \right\|_{\infty} $ can 
then
be bounded by using
the assumption on $\lambda$ in Theorem~\ref{thm:stat},
and the second term 
$\left\| \partial \phi( \ten{X}_{\ip{i}} ) \right\|_{\infty}$ in above inequality.
%(\ref{eq:tmp})
can be bounded by using Lemma~\ref{lem:app2}.
As a result,
the assumption on $\| [ \nabla f( \tilde{\ten{X}} ) ]_{\ip{i}} \|_{\infty}$ can
be removed.

\vspace{5px}
\hrule
\vspace{10px}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q11.}
\textit{It would be useful to provide a small proof sketch or proof idea below Theorem 14 
	(Theorem~\ref{thm:stat} in this revision)
	to help with
	readability.}

\vspace{5px}
\noindent
\textbf{Reply.}
As suggested,
a sketch of the proof for Theorem~\ref{thm:stat}
is added  in this revised version.
%The proof is performed with three main steps and the general idea this proof is inspired by~\citep{loh2015regularized}.  However, different math tools are used by \citep{loh2015regularized} and ours, since \cite{loh2015regularized} focuses on sparse vectors, of which each dimension is separable, and we work with overlapped tensor regularization, where singular values are coupled with each other.



\subsubsection*{Experiments}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q12.1.}
\textit{In figure 3, 
	the statistical error is a flat line which is rather surprising. 
	What this seems to be indicating is that even with better optimization, 
	this error is not going down. 
	Can the authors comment on this? }

\vspace{5px}
\noindent
\textbf{Reply.}
In 
%Section~5.1.3 (of 
the previous version,
the statistical error is defined as the RMSE between a critical point $\tilde{\ten{X}}$ returned by
NORT on convergence
and the
underlying ground-truth $\ten{X}^*$
(i.e.,
$\| \tilde{\ten{X}} -\ten{X}^* \|_{F}$).
%while the optimization error is measured as the RMSE between iterate $\ten{X}_t$ and the globally optimal solution $\dot{\ten{X}}$ of \eqref{eq:pro} (i.e., $\| \ten{X}_t - \dot{\ten{X}} \|_{F}$).
Thus,
it does not depend on $t$,
and is a flat line.
%\footnote{$\surd$ yes.  the previous plot follows Figure 1 in~\citep{loh2015regularized}.  However, as suggested by the reviewer, adding $_t$ is more proper for us.  *** so in the prev ver, u did not plot $\| \ten{X}_t - \ten{X}^* \|_{F}$ as the statistical error?}

As suggested by the reviewer,
we now define the statistical error
as $\| \ten{X}_t - \ten{X}^* \|_{F}$
in this revised version.
As can be seen from the
updated
figures in Section~\ref{sec:quacri},
the statistical error of $\ten{X}_t$ decreases
as $t$ becomes larger.
%However, the statistical error is generally larger than the optimization error since the recovery can be guaranteed but may not be exact, i.e., $\| \tilde{\ten{X}} - \dot{\ten{X}} \|_F$ can be small but may not be zero.

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q12.2.}
\textit{Also, how were these different instances initialized?}

\vspace{5px}
\noindent
\textbf{Reply.}
%\footnote{+qm+ add back to the main text?}
This is now clarified in the first paragraph in Section~\ref{sec:quacri}.
Specifically, we set
$\ten{X}_0 = \ten{X}_1  = \sum\nolimits_{i = 1}^D \big( \vect{u}^i ( \vect{v}^i
)^{\top} \big)^{\ip{i}}$,
where elements in $\bm{u}^i$'s and $\bm{v}^i$'s follow $\mathcal{N}(0, 1)$.
%Initialized factors $\{ \bm{U}_i, \bm{V}_i \}$'s are randomly initialized
%using Gaussian $\mathcal{N}(0, 1)$.
%Figure~\ref{fig:syn:staterr_vs_opterr} has been updated.\footnote{*** still
%straight line?}

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q12.3.}
\textit{In terms of statistical
	error, it appears that the initialization seems good enough.}

\vspace{5px}
\noindent
\textbf{Reply.}
Sorry for causing such a misunderstanding.
Please see our reply to Q12.1.
From Figure~\ref{fig:syn:staterr_vs_opterr} in the revised version,
it can be seen that
the statistical error decreases significantly during iterating.


\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q12.4.}
\textit{What is the statistical error if we
	predict the all zeros tensor (or a constant tensor)?}

\vspace{5px}
\noindent
\textbf{Reply.}
As suggested,
instead of using a low-rank tensor,
we use an all-one tensor as the ground-truth.
The remaining setup is the same as in Section~\ref{sec:quacri}.
The 
figure
below 
shows 
the statistical and optimization errors.
As can be seen,
the observations are the same as for
Figure~\ref{fig:syn:staterr_vs_opterr} in the revised version.
It can be seen that
the both statistical and optimization errors decrease significantly during iterating.
The statistical error is generally larger than the 
optimization error
and does not 
converge to zero.

\begin{figure}[H]
\centering
\subfigure[LSP.]{\includegraphics[width=0.32\textwidth]{figures/rebuttal/stat-reg2-constant}}
\qquad
\subfigure[capped-$\ell_1$.]{\includegraphics[width=0.32\textwidth]{figures/rebuttal/stat-reg1-constant}}
\vspace{-10px}
\begin{center}
\begin{minipage}{0.8\textwidth}
Statistical error (in red) and optimization error (in black) versus the number of NORT iterations on
an all-one tensor 
(with $\hat{c} = 400$). 
Both 
the optimization and statistical error curves are averaged from $20$ runs of NORT with different random seeds.
\end{minipage}
\end{center}
\end{figure}

\vspace{5px}
\hrule 
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q13.1}
\textit{In the synthetic data experiments, the results are only shown for a fixed noise level (with very
	low variance) and 
	50\% of data, with 3rd order tensors.
I think it would be quite useful to see
	ablation studies across these three axes: varying the noise level, the amount of data as well as
	the order (and dimension) of the tensor to understand how much better is the proposed algorithm as
	compared with benchmark.
Currently, I am unable to verify if the proposed algorithm’s gains are
	only to be realized in the high signal to noise regime, or only in lower order tensors or are
	these claims much more general?}

\vspace{5px}
\noindent
\textbf{Reply.}
First, please note that ``using 50\% of the training data" means that we use 50\% of the observed training entries 
(which is very few,
as can be seen from Table~\ref{tab:synperf:large}),
not 50\% of all tensor entries.


As suggested,
in 
this revised version,
we have 
added ablation studies
on the 
noise level (Section~\ref{sec:exp:obvnsy}),
number of observations
(Section~\ref{sec:exp:obvnsy}),
tensor rank (Section~\ref{sec:orderrank}),
and tensor order (Section~\ref{sec:orderrank}).
As can be seen 
from these newly added experiments,
the proposed NORT
achieves the same testing performance as GDPAN,
but NORT is much more efficient than GDPAN 
at various noise levels (Figure~\ref{fig:time:noisy}),
numbers of observations (Figure~\ref{fig:time:obv}),
different tensor orders (Figure~\ref{fig:time:syn-order})
and ground-truth ranks (Figure~\ref{fig:time:syn-rank}).

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q13.2}
\textit{Similar thing for the setup in Section 5.2.1 where the Gaussian noise has variance 0.01. I would
	request the authors to perform a detailed study here with varying noise levels, and showing that
	the gains still hold in the high noise regimes?}

\vspace{5px}
\noindent
\textbf{Reply.}
As suggested, 
in this revised version,
we have added new experiments 
in Section~\ref{sec:image}.
The gains still hold in the high noise regimes.
However,
the recovery performance of all methods are not good.
%We copy results and analysis in Section~\ref{sec:image} here
%for a easy check.

%{
%\it
%\noindent
%We compare 
%NORT with the PA-APG and RP,
%which are
%the best one in Table~\ref{tab:colorimg}
%from convex and factorization category respectively,
%under different noise level.
%The testing RMSEs
%are reported in Table~\ref{tab:colorimg:nlvl}
%(copied as below table).
%We can see 
%that 
%the testing RMSEs of all methods 
%generally get large as the noise level $\sigma$ becomes higher.
%NORT gets relatively
%lower testing RMSEs when $\sigma = 0.01$ and $0.001$.
%This is because 
%the natural images may not be exactly low-rank,
%then adaptive penalization of singular values 
%can better preserve their spectrum.
%Such an observation is also previously made in \citep{yao2018large,lu2016nonconvex} for nonconvex regularization on 
%image matrices.
%However,
%when the noise level becomes
%really high,
%i.e.,
%pixels are in $[0, 1]$ and $\sigma = 0.1$,
%while NORT can still be better
%the testing RMSE of all methods are not small.
%
%\begin{table}[H]
%	\centering\it
%%	\caption{}
%	\centering
%	Testing RMSEs on image \textit{Tree}.
%	The percentage followed by the marker 
%	$\uparrow$ indicates the relatively increase of 
%	testing RMSE compared with NORT.
%	
%	\small
%%	\vspace{-8px}
%	\begin{tabular}{c | c|  c | c | c}
%		\toprule
%		\multicolumn{2}{c|}{noise level $\sigma$} & 0.001                      & 0.01                       & 0.1                        \\ \midrule
%		convex     & PA-APG       & 0.0149 (35.8\% $\uparrow$) & 0.0488 (24.6\% $\uparrow$) & 0.0585 (18.6\% $\uparrow$) \\ \midrule
%		factorization & RP           & 0.0139 (26.0\% $\uparrow$) & 0.0575 (15.6\% $\uparrow$) & 0.0388 (10.1\% $\uparrow$) \\ \midrule
%		nonconvex   & NORT         & 0.0110                     & 0.0386                     & 0.0297                     \\ \bottomrule
%	\end{tabular}
%\end{table}
%}

%add experiments
%\footnote{+qm+ add in Figure~\ref{fig:noisy}}
%\footnote{+qm+ may need to update Figure~\ref{fig:syn-order} and \ref{fig:syn-rank} as well.}


\subsubsection*{Minor points}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q14.}
\textit{Provide a definition of tensor rank in the preliminaries}

\vspace{5px}
\noindent
\textbf{Reply.}
As suggested,
we added a definition of tensor rank at the beginning of
Section~\ref{sec:ten:reg}
in this revised version.

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q15.}
\textit{Page 5: The authors mention that the overlapped nuclear norm minimization is guaranteed to find
	low rank tensors, could the authors please elaborate a bit more on the exact guarantee here?}

\vspace{5px}
\noindent
\textbf{Reply.}
In this revision,
we elaborated on
these guarantees at the end of Section~\ref{sec:ten:reg}.

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q16.}
\textit{Below eq.(9), the paper mentions that there can be instances where prox step for each $g_i$ is
	easily obtained but not for the combination -- it would be useful to provide an example for this
	to help the reader appreciate this point better.}

\vspace{5px}
\noindent
\textbf{Reply.}
As suggested,
we have added ``simultaneously sparse and low-rank'' as an example 
under \eqref{eq:compopt}
to illustrate this point.

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q17.}
\textit{It would be useful to highlight what was special about the 
	$M = 3$ case handled in the conference
	version which was hard to transfer to the higher $M$ case in this paper. 
	Also, it would be useful to
	provide an intuitive idea of the algorithm by explaining it for the 
	$M = 3$ case in this paper as
	well.}

\vspace{5px}
\noindent
\textbf{Reply.}
The algorithm
can be used with arbitrary $M$ including the case both $M = 3$ and $M > 3$.
It is Proposition~3.2
in the conference version,
not the algorithm, 
that limits us to $M = 3$.
Without such a Proposition,
the algorithm can suffer from expensive computation cost,
and thus no efficiency advantage over the simple use of the PA algorithm.
%We have also elaborated this point after \eqref{eq:l_gradient} 
%in the journal version.

%As for  ,
Specifically,
when mapping the vector $\bm{v}_p$ back to a matrix,
we do not need to take a special treatment on the size of matrix.
The reason is that
$\bm{v}_p$ has $I_i I_j$ elements
and we just need to map it back to a matrix of size $I_i \times I_j$.   
Thus, we do not have parameters 
for the \textit{mat} operation in the conference version.
However,
when $M > 3$,
$\bm{v}_p$ has $I^{\pi}/I^i$ elements,
we need to check 
whether ideas used in the conference version 
can still be done in a similar way.
As a result,
we have two more parameters
for the \textit{mat} operation in the journal version,
which customize reshaping matrix to a proper size.

In this revised version,
we added the above justifications and make this point clearer 
after Proposition~\ref{pr:mulv}.




\section*{To Reviewer \#3}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q1.}
\textit{I would suggest avoiding sloppy/ambiguous phrases that might be misleading. For instance,
	the authors state under the usual smoothness assumption or KL condition, but they don't point out
	the smoothness assumption on which quantity in a few places.}

\vspace{5px}
\noindent
\textbf{Reply.}
Sorry for causing such a confusion.
We have checked the whole paper,
and make it clear that
%In the whole paper,
the smoothness assumption is always imposed on 
the loss (i.e., $f$),
and the KL condition is imposed on the whole 
training objective (i.e., $F_{\tau}$).

%The KL condition cannot replace the smoothness assumption
%as there are example functions which are smooth but fail to meet KL condition.
%Please check Section~4.3 of~\citep{bolte2010characterizations}.
%In
%this revision,
%to avoid such a confusion,
%we have
%\begin{itemize}[leftmargin=*]
%\item added in the beginning part of Section~\ref{sec:convana}
%that smooth is always assumed.
%
%\item elaborated more on KL condition and clarified its connections with smooth assumption
%in Section~\ref{sec:conv:kl} around Definition~\ref{def:kl}.
%\end{itemize}
%We have also double checked other phrases in this revision.

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q2.}
\textit{The paper could be better organized to reduce confusion or misunderstanding. In the
	introduction of the setting, a few settings are introduced. The readers might have a feeling of a
	jumping mindset from convex to nonconvex and then back to convex again. For example, PA is first
	introduced as for convex g but then clarified that it has been extended to nonconvex g. I think it
	would be better to say that the first time when introducing it that it could be nonconvex..}

\vspace{5px}
\noindent
\textbf{Reply.}
To reduce the jump between convex and nonconvex parts,
at the beginning of Section~\ref{sec:pa}
in this revised version,
we only state the form of the optimization problem 
\eqref{eq:compopt}
that can be solved by the PA algorithm.
Discussion of the convex and nonconvex parts are moved to the end of Section~\ref{sec:pa}.
%% when stating existing convergence results of PA algorithm.
For presentation of the proposed method
in Section~\ref{sec:proalg},
we only consider the case where $f$ is smooth and $g$ is nonconvex and nonsmooth.
%These assumptions do not change in the sequel. 

\vspace{5px}
\hrule
\vspace{10px}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent
\textbf{Q3.}
\textit{Some notations are not well defined. For instance, in equation (7), $\sigma_i(x)$ is first
	used to denote the singular values of X, but it was never formally introduced. Another example is
	that O is first introduced in equation (13), but the author never defined it. In Algorithm 1, O is
	never defined or set as the input to the algorithm, but it is used, nevertheless, in the
	algorithm.}

\vspace{5px}
\noindent
\textbf{Reply.}
In this revision,
we have added definitions for 
$\sigma_i(\bm{X})$ at the notation part of Section~\ref{sec:intro},
described $\ten{O}$ under \eqref{eq:pro},
and add $\SO{\ten{O}}$ at the input of Algorithm~\ref{alg:compp3}.
We have also double checked other 
parts of this submission as well.


